Empirical Investigation of Neural Symbolic Reasoning Strategies

Neural reasoning accuracy improves when generating intermediate reasoning steps. However, the source of this improvement is yet unclear. Here, we investigate and factorize the benefit of generating intermediate steps for symbolic reasoning. Specifically, we decompose the reasoning strategy w.r.t. step granularity and chaining strategy. With a purely symbolic numerical reasoning dataset (e.g., A=1, B=3, C=A+3, C?), we found that the choice of reasoning strategies significantly affects the performance, with the gap becoming even larger as the extrapolation length becomes longer. Surprisingly, we also found that certain configurations lead to nearly perfect performance, even in the case of length extrapolation. Our results indicate the importance of further exploring effective strategies for neural reasoning models.

==> body/2_related_work.tex <==
\section{Related Work}
\label{related_work}
As for output strategies, some studies trained the models to generate reasoning steps and a conclusion derived from them at once~\cite{Nye2021,Lewkowycz2022,Wei2022,Kojima2022,Wang2022,Recchia2021}, some generated 
a single reasoning step given the input and iterated this process until achieving a conclusion~\cite{Sanyal2022,Picco2021,Tafjord2021}, and others iteratively generated sub-goals as well as reasoning steps~\cite{Liang2021,Shwartz2020}.
As for chaining strategies, some studies used a backward chaining process~\cite{Picco2021,DBLP:conf/nips/Rocktaschel017,DBLP:conf/aaaiss/CingilliogluR19}, and others adopted exhaustive searches~\cite{Tafjord2021,Liang2021,DBLP:journals/corr/abs-2205-12443}.
\citet{Gontier2020} compared the chaining strategies and concluded that models that \textit{didn't} generate reasoning steps had better generalization performance than models that did.
In a similar vein, we investigate the combinations of chaining and decoding strategies, and find that both substantially affect the symbolic reasoning performance of neural seq2seq learners.

==> tables/compare.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lp{4 cm}}
\multicolumn{2}{l}{Question: \texttt{A=1, D=3+A, B=2+A, C=5+B, C?}} \\
\toprule
Chain strategy & Reasoning steps \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2} 
Shortest & \textcolor{gray}{(omit D)} \\ 
&\texttt{B=2+A, B=2+1, B=3,} \\
&\texttt{C=5+B, C=5+3, C=8} \\ 
\cmidrule(lr){1-1} \cmidrule(lr){2-2} 
Exhaustive & \texttt{D=3+A, D=3+1, D=4,}\\
&\texttt{B=2+A, B=2+1, B=3,}\\
&\texttt{C=5+B, C=5+3, C=8} \\
\bottomrule
\end{tabular}
\caption{Illustration comparing the shortest-path and exhaustive strategies in terms of granularity of inference. In this table, ``(omit D)'' denotes that the model omits the computation of variable D.}
\label{table:compare}
\end{table}
